Reparo: Publicly Verifiable Layer to Repair Blockchains

Although blockchains aim for immutability as their core feature, several instances have exposed the harms with perfect immutability. The permanence of illicit content inserted in Bitcoin poses a challenge to law enforcement agencies like Interpol, and millions of dollars are lost in buggy smart contracts in Ethereum. A line of research then spawned on Redactable blockchains with the aim of solving the problem of redacting illicit contents from both permissioned and permissionless blockchains. However, all the existing proposals follow the build-new-chain approach for redactions, and cannot be integrated with existing systems like Bitcoin and Ethereum. We present Reparo, a generic protocol that acts as a publicly verifiable layer on top of any blockchain to perform repairs, ranging from fixing buggy contracts to removing illicit contents from the chain. Reparo facilitates additional functionalities for blockchains while maintaining the same provable security guarantee; thus, Reparo can be integrated with existing blockchains and start performing repairs on the pre-existent data. Any system user may propose a repair and a deliberation process ensues resulting in a decision that complies with the repair policy of the chain and is publicly verifiable. Our Reparo layer can be easily tailored to different consensus requirements, does not require heavy cryptographic machinery and can, therefore, be efficiently instantiated in any permission-ed or -less setting. We demonstrate it by giving efficient instantiations of Reparo on top of Ethereum (with PoS and PoW), Bitcoin, and Cardano. Moreover, we evaluate Reparo with Ethereum mainnet and show that the cost of fixing several prominent smart contract bugs is almost negligible. For instance, the cost of repairing the prominent Parity Multisig wallet bug with Reparo is as low as 0.000000018% of the Ethers that can be retrieved after the fix.

==> bitcoin.tex <==



==> graph1.tex <==
\begin{tikzpicture}                                                            
  \begin{axis}[
  width=1.2\textwidth,
    height=11em,
    ymin=80,  
    bar width=3mm,
    xtick=data,
    xmin=0.3,
    xmax=5.7,
    ymax=5,
    ymin=-0.5,
    ybar=0,
    extra y ticks       = 0,
   % ylabel={Overhead},
    xlabel={\footnotesize Chain size (in \# of blocks)},
    yticklabel=\scriptsize \pgfmathparse{1*\tick}\pgfmathprintnumber{\pgfmathresult}\,\%,
    xticklabel=\scriptsize \pgfmathparse{1*\tick}\pgfmathprintnumber{\pgfmathresult}0K,
    yticklabel style={/pgf/number format/.cd,fixed,precision=2}
        ]  \addplot
coordinates {
(1, 3.053083427557031)
(2, 2.9673926381325466)
(3, 3.7991830096397026)
(4, 1.0473486742365898)
(5, 0)};
%\draw[thin] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0);
  \end{axis}
\end{tikzpicture}

\caption{}

==> graph2.tex <==
\begin{tikzpicture}
  \begin{axis}[
  width=1.2\textwidth,
    height=11em,
    ymin=80,  
    bar width=3mm,
    xtick=data,
    xmin=0.5,
    xmax=5.5,
    ymax=5,
    ymin=-0.5,
    ybar=0,
    extra y ticks       = 0,
   % ylabel={Overhead},
    xlabel={\footnotesize $\#$ of redactions in the chain},
    yticklabel=\scriptsize \pgfmathparse{1*\tick}\pgfmathprintnumber{\pgfmathresult}\,\%,
    xticklabel=\scriptsize \pgfmathparse{1*\tick}\pgfmathprintnumber{\pgfmathresult}K,
    yticklabel style={/pgf/number format/.cd,fixed,precision=2}
        ]
  \addplot
coordinates {
(1, 1.3070767719031349)
(2, 0.8628298316230483)
(3, 1.9483735313250665)
(4, 1.7370226878977915)
(5, 2.9612391807180543)
};
%\draw[thin] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0);
  \end{axis}
\end{tikzpicture}

\caption{}

==> graph3.tex <==
\begin{tikzpicture}
  \begin{axis}[
  width=1.2\textwidth,
    height=11em,
    ymin=80,  
    bar width=3mm,
    xtick=data,
    xmin=10,
    xmax=60,
    ymax=5,
    ymin=-0.5,
    ybar=0,
    extra y ticks       = 0,
    %ylabel={Overhead},
    xlabel={\footnotesize Voting period $\ell$},
    xticklabel=\scriptsize \pgfmathparse{1*\tick}\pgfmathprintnumber{\pgfmathresult},
    yticklabel=\scriptsize \pgfmathparse{1*\tick}\pgfmathprintnumber{\pgfmathresult}\,\%,
    yticklabel style={/pgf/number format/.cd,fixed,precision=2}
        ]
  \addplot
coordinates {
%(10, 0.8395723484928953)
(15, 0)
(20, 0)
(25, 0)
(30,0)
(35,1.6217981388567646)
(40,1.2889899688943318)
(45,2.4215612763945873)
(50,1.5354370027936013)
(55,3.3150705290616647)
%(60,0)
};
%\draw[thin] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0);
  \end{axis}
  
  \end{tikzpicture}

\caption{}

==> newprotocol.tex <==
\section{Our Edit Layer}\label{sec:editing-new}

In this section we show how to extend a given immutable blockchain protocol $\Blk$ (as described in Section~\ref{sec:abstraction}) into an \emph{editable} blockchain protocol $\Blk'$ which allows to make \emph{redactions} and \emph{state updates} on the chain.



\subsection{Edit Layer Description}\label{sec:editable-newnew}

Our edit layer is formally described in Fig.~\ref{fig:newprotocol}. It allows the redaction of data from the blockchain and/or special changes in the current state of the chain. 
%Note that the data that is allowed to be redacted must not affect the current state of the chain, and hence are also referred to as stateless edits. 

We add an additional category of parties apart from users and miners to the set of parties involved in our protocol, namely \emph{deciders}. Note that the categories are \emph{not} mutually exclusive, e.g., a user can also be a decider and/or a miner.


 Consider a block $B:= \langle \header, \data \rangle$; a redaction replaces the data $\data \in\{0,1\}^*$ with new data $\data' \in\{0,1,\bot\}^*$, where some portion of the data have been redacted, i.e., for all data points $\data_i' \in \data'$ and $\data_i \in \data$, we have $\data'_i \in \{\data_i,\bot\}$. This ensures that no data point has been modified into a different data point. 
%
Any other edit operation acts as any other type of message that changes the current state of the blockchain. In contrast to normal messages, e.g. such as Alice send some coins to Bob, a state-update message can alter the current balances of Alice and Bob arbitrarily.



Both redactions and state-updates can be proposed by users. A redaction proposal $\rp = \langle \pt, \data' \rangle$ consists of a block-pointer $\pt$ and the new data $\data'$ (with some portion of the old data removed). A state-update proposal $\sprop$ is a (set of) message(s) that describes the desired state change. 

Both types of proposals are collected by miners and deciders. The deciders then use a decision protocol to deliberate whether a
proposal should be accepted or not. The protocol outputs their final decision in the form of a witness. Miners then should add this witness into the header data of the next created block. For concreteness, one can consider the same decision process as in~\cite{deuber2019redactable}, where deciders (i.e., the miners themselves) add their votes to the header data $\hdata$ of their newly created blocks before broadcasting it to the network; the witness can then be easily ``extracted'' from the header data of all the blocks during the deliberation period, by simply counting how many votes supported the proposal.

In case of a redaction, the witness $\redactwit = \langle \pt, G(\data'), b, \pf \rangle$ consists of a block-pointer $\pt$ and the pointer to the new data $\data'$, the decision bit $b$, and a proof $\pf$ which allows to validate the decision (e.g., verifiable vote count). Since the redaction is stateless, $\redactwit$ need not contain any state information.
For state-updates the witness $\statewit = \langle \sprop, b, \pf \rangle$ simply consists of the proposed state-change $\sprop$, the decision bit $b$ and a proof $\pf$ which allows to validate the decision. Note that for any proposal $\prop$, we require the witness proof $\pf$ to be unforgeable, i.e., it should be infeasible for an adversary to produce a valid proof $\pf'$ for a proposal $\prop$ that was \emph{not} accepted by the protocol. 

We assume that there is a predicate $\checkApproval(\prop, \policy)$ which determines if a proposal $\prop \in \{\sprop,\rp\}$ is approved. It takes as input a proposal $\prop$ (that can be a redaction proposal or a state update), and a policy $\policy$. The policy here dictates the constraints of redaction/state update, e.g., what is the duration of the deliberation period, what type of data can be redacted, what changes in the state are allowed. The predicate outputs $1$ if the proposal $\prop$ complies by the policy $\policy$.

\TODOB{We need to say somewhere that the policy does not allow to redact header data, and that state update cannot change system parameters such as chain difficulty and etc. In the proofs I'm calling as ``valid'' policy to denote  policies that dictates rules that enforce the edits based on the restrictions mentioned previously.}

%We note that a redaction proposal $\rp = \langle \pt, \data' \rangle$ is \emph{not} allowed to change the state of the chain, i.e., let $\state$ be the state defined by the chain up to (and including) block $\pt$, and let $\state'$ be the state where the data of block $\pt$ is replaced by $\data'$; then the redaction proposal $\rp$ is valid iff $\state = \state'$.


%\paragraph{Intuition} On a high level the $\layer$ classifies the users of system as \emph{miners, deciders} and \emph{users}. Any \emph{user} is allowed to make an edit request that can either purge some data from a block or perform an edit operation that changes the state of the system from thereon. A \emph{miner} collects all such requests from the network and validates them before adding them to the candidate pool of candidate blocks. If a request is approved, the \emph{miner} performs the edit operation, be it purging of data or a stateful edit operation. In case of stateful edits, the \emph{miner} also needs to update the state of the system starting from the position the edit was performed until the point the request has been approved. To do this, we introduce the $\layer$ state transition function $\transition^\star: \bit^* \times \bit^* \times \bit^* \rightarrow \bit^*$ that takes as inputs the latest approved request, the chain and the new inputs from the network and returns the updated state of the system until that point in time. $\transition^\star$ takes into account the all the previous state updates that are reflected onto the chain already. \emph{Decider} deliberate on a proposed request and vote for the request to be approved or not. If the votes satisfy the edit policy $\policy$ of the system, then the request is considered to be approved and a decision $d$ is posted on the blockchain that helps \emph{miners} perform the edit operation and also future users in validation of chain edits.

%\TODOD{We assume that users/deciders get their chain from miners.}
\floatstyle{boxed}
\restylefloat{figure}


\begin{figure*}
	
	The protocol $\layer$ has access to a blockchain protocol $\Blk$. The communication with $\Blk$ happens through the interfaces described in Section~\ref{sec:abstract-newnew}. The protocol is parametrized by a policy $\policy$ that specifies the duration (in slot numbers) of the deliberation period, what type of data can be redacted, and what changes in the state are allowed. We formally describe the $\layer$ protocol below.
	
\begin{description}
	\item[Initialisation (miner/decider).] Initialize the \emph{proposal pool} to be empty by setting $\rcbpool \gets \emptyset$. 


	\item[Proposal.] Any user can propose either a redaction or a state update as follows.
	\begin{itemize}
		\item \emph{Redaction:} The user creates a redaction proposal $\rp = \langle \pt, \data' \rangle$ and broadcasts it to the network by calling $\Blk.\broadcast(\rp)$.
		\item \emph{State Update:} The user creates a state-update proposal $\sprop$ and broadcasts it to the network by calling $\Blk.\broadcast(\sprop)$.
	\end{itemize}

	\item[Update proposal pool.] The miners/deciders periodically collect all valid proposals and add them to the proposal pool. They remove a proposal from the pool if there is a witness for the proposal in the stable part of the chain.

	\item[Deliberation Process (decider/miners).] Once a new proposal $\prop \in \{\rp,\sprop\}$ is collected the deciders collectively start the decision protocol. This protocol outputs (i.e., broadcasts) a witness $w \in \{\redactwit,\statewit\}$ of their decision. The miners then add the new witness into the header data $\hdata$ of the next new block.

	\item[Editing the chain (miners).] The miners are responsible to act on positive decisions for redaction or state updates as follows.	
	\begin{itemize}
		\item \emph{Redaction:} A redaction proposal $\rp = \langle \pt, \data' \rangle$ is enacted as soon as there is a positive redaction witness of the form $\redactwit:= \langle \pt, G(\data'),1, \pf \rangle$ in the stable part of the chain $\chain$. The miner replaces the $\data$ of the block pointed by $\pt$ by the new data $\data'$.
	
		\item \emph{State Update:} A state update proposal $\sprop$ is enacted as soon as a positive state update witness $\statewit := \langle \sprop, 1, \pf \rangle$ is found in the block header data $\hdata$. No special action from the miners is required.
	\end{itemize}		
	

	\item[Chain validation (miners).] The chain validation procedure begins by validating from the genesis block. It works by updating $\Blk.\chainValid$ to handle different edit operations as follows:
	\begin{itemize}
		\item \emph{Witnesses:} $\Blk.\chainValid$ is updated to accept witnesses in the block header-data, $\hdata$. A witness $w \in \{\redactwit,\statewit\}$ is valid if the proposed change is approved according to $\checkApproval$ (cf. Section~\ref{sec:editable-newnew}) and if the proof $pf$ is valid, i.e., the witness is the output of the correct decision protocol.  
	
		\item \emph{State-Update:} $\Blk.\chainValid$ is updated to incorporate state-changes implied by valid state-update witnesses. The state change is performed as was originally done by miners.
		
		\item \emph{Redaction:} Consider a block $B:= \langle \header, \data \rangle$. To accommodate redactions, $\Blk.\chainValid$ is updated to check if either the pointer of $\data$ is equal to the data-pointer $G(\data)$ that is stored in the $\header$ or for the (starting from the head of the chain) first positive redaction witness $\redactwit := \langle \pt, g, 1, \pf \rangle$ where $\pt$ points to $B$ it holds that $G(\data)=g$.
		\item Finally, ensure that all edit operations - both redactions and state updates - that have an approved witness $w$ on the chain have been performed. This check can be performed on the fly as we validate blocks from the genesis.
	\end{itemize}

\end{description}

	\caption{Editable blockchain protocol $\Blk'_\policy$ with $\layer$ on $\Blk$}
	\label{fig:newprotocol}
\end{figure*}




==> picture.tex <==
\begin{figure*}[t]
\begin{minipage}{0.48\linewidth}
	\centering
	\resizebox{\linewidth}{!}{
	\begin{tikzpicture}[every node/.style={font=\tiny}]
		
	    \node (n1) []  {};
	    
		%boxes at the top	
		\node (b1) [block, below of = n1,minimum width=4.5em] {\huge$B_j$};
		\node (b2) [block, right of = b1, xshift=4em, minimum width=4.5em] {};
		\node (b3) [block, right of = b2, xshift=4em,minimum width=4.5em] {\Large \textcolor{red}{$H(\candidateblk_j)$}};
		\node (b4) [block, right of = b3, xshift=4em,minimum width=4.5em] {\Large $H(\candidateblk_j)$};
		\node (b5) [block, right of = b4, xshift=4em,minimum width=4.5em] {};
		\node (b6) [block, right of = b5, xshift=4em,minimum width=4.5em] {\Large $H(\candidateblk_j)$};
		\node (b7) [block, right of = b6, xshift=4em,minimum width=4.5em] {\Large $H(\candidateblk_j)$};

		\draw [arrow,dashed] ([yshift=0.25cm]b2.west) -- ([yshift=0.25cm]b1.east);
		
		\draw [arrow] ([yshift=-0.25cm]b2.west) -- ([yshift=-0.25cm]b1.east);
		\draw [arrow,dashed] ([yshift=0.25cm]b3.west) -- ([yshift=0.25cm]b2.east);
		
		\draw [arrow] ([yshift=-0.25cm]b3.west) -- ([yshift=-0.25cm]b2.east);
		
		\draw [arrow,dashed] ([yshift=0.25cm]b4.west) -- ([yshift=0.25cm]b3.east);
		\draw [arrow] ([yshift=-0.25cm]b4.west) -- ([yshift=-0.25cm]b3.east);
			\draw [arrow,dashed] ([yshift=0.25cm]b5.west) -- ([yshift=0.25cm]b4.east);
		
		\draw [arrow] ([yshift=-0.25cm]b5.west) -- ([yshift=-0.25cm]b4.east);
		\draw [arrow,dashed] ([yshift=0.25cm]b6.west) -- ([yshift=0.25cm]b5.east);
		\draw [arrow] ([yshift=-0.25cm]b6.west) -- ([yshift=-0.25cm]b5.east);
		\draw [arrow,dashed] ([yshift=0.25cm]b7.west) -- ([yshift=0.25cm]b6.east);
		\draw [arrow] ([yshift=-0.25cm]b7.west) -- ([yshift=-0.25cm]b6.east);

		
		%text at the top
		\node (nt1) at ($(b4.west)!0.5!(b7.east)$) {};

\draw [decorate,decoration={brace,amplitude=10pt,raise=25pt},xshift=0pt,yshift= 4cm]
(b4.west) -- (b7.east) node [black,midway,yshift=2cm] 
{\huge Voting period ($\ell$)};

\draw [decorate,decoration={brace,amplitude=10pt,raise=25pt},yshift= 4cm]
(b3.west) -- (b3.east) node (propose) [black,midway,yshift=2cm] 
{\huge propose $\candidateblk_j$};


%\draw [decorate,decoration={brace,amplitude=10pt,raise=25pt},yshift= 4cm]
%(b2.west) -- (b2.east) node [black,midway,yshift=2cm] 
%{\huge Block $B_j$};



\node [cloud, above of =b2, yshift = 4cm,draw,cloud puffs=10,cloud puff arc=120, aspect=2, inner ysep=3.6em](cl) { };
\node (intro4) at ($(cl.east)$){};
%\draw[arrow, line width=1.2pt] (intro2) to[out=-160,in=0] (intro4);


\node (cl1) [block, above of =cl, yshift =0.5cm]{\huge $B^\star_k$};
\node (cl2) [block, right of =cl1,xshift = 1cm,yshift =-0.5cm]{\huge $B^\star_l$};
\node (cl3) [left of =cl1,xshift = -1cm,yshift =-0.5cm]{\huge $\rcbpool$};
\node (cl4) [block, left of =cl,xshift = -0.5cm,yshift =-0.4cm]{\huge $B^\star_n$};
\node (cl5) [block, dashed, right of =cl,xshift = 0.2cm,yshift =-0.4cm]{\huge \textcolor{red}{$\candidateblk_j$}};

\draw [arrow,dashed] ([xshift=-2em]propose.north east) to[out=100,in=0] ([yshift=1.2em,xshift=0.5em]cl5.south east);


	\end{tikzpicture}
	}
\subcaption{Proposing a redaction $\candidateblk_j$ for the block $B_j$}
\label{fig:abstract_before_redaction}
\end{minipage}
\hfill\vline\hfill
\begin{minipage}{0.48\linewidth}
	\centering
	\resizebox{\linewidth}{!}{
	\begin{tikzpicture}[every node/.style={font=\tiny}]
		
	    \node (n1) []  {};
	    
		%boxes at the top	
		\node (b1) [block, below of = n1,minimum width=4.5em] {\huge \textcolor{red}{$B^\star_j$}};
		\node (b2) [block, right of = b1, xshift=4em,minimum width=4.5em] {};
		\node (b3) [block, right of = b2, xshift=4em, minimum width=4.5em] {\Large \textcolor{red}{$H(\candidateblk_j)$}};
		\node (b4) [block, right of = b3, xshift=4em,minimum width=4.5em] {\Large $H(\candidateblk_j)$};
		\node (b5) [block, right of = b4, xshift=4em,minimum width=4.5em] {};
		\node (b6) [block, right of = b5, xshift=4em,minimum width=4.5em] {\Large $H(\candidateblk_j)$};
		\node (b7) [block, right of = b6, xshift=4em,minimum width=4.5em] {\Large $H(\candidateblk_j)$};
		
		\node (cross) [cross out, inner sep = 0.6em,draw=black,yshift=0.25cm,line width = 1.3pt] at ($(b1.east)!0.5!(b2.west)$){};
		%\node (b8) [block, right of = b7, xshift=2cm] {};
		%\node (b9) [block, right of = b8, xshift=2cm] {};
		%dotted lines / arrows between the boxes
		%\draw [arrow, dashed, very thick] (b2) -- (b1);
		\draw [arrow,dashed] ([yshift=0.25cm]b2.west) -- ([yshift=0.25cm]b1.east);
		
		\draw [arrow] ([yshift=-0.25cm]b2.west) -- ([yshift=-0.25cm]b1.east);
		\draw [arrow,dashed] ([yshift=0.25cm]b3.west) -- ([yshift=0.25cm]b2.east);
		
		\draw [arrow] ([yshift=-0.25cm]b3.west) -- ([yshift=-0.25cm]b2.east);
		%%\draw [arrow,dashed] ([yshift=0.25cm]b4.west) -- ([yshift=0.25cm]b3.east);
		
		\draw [arrow,dashed] ([yshift=0.25cm]b4.west) -- ([yshift=0.25cm]b3.east);
		\draw [arrow] ([yshift=-0.25cm]b4.west) -- ([yshift=-0.25cm]b3.east);
			\draw [arrow,dashed] ([yshift=0.25cm]b5.west) -- ([yshift=0.25cm]b4.east);
		
		\draw [arrow] ([yshift=-0.25cm]b5.west) -- ([yshift=-0.25cm]b4.east);
		\draw [arrow,dashed] ([yshift=0.25cm]b6.west) -- ([yshift=0.25cm]b5.east);
		\draw [arrow] ([yshift=-0.25cm]b6.west) -- ([yshift=-0.25cm]b5.east);
		\draw [arrow,dashed] ([yshift=0.25cm]b7.west) -- ([yshift=0.25cm]b6.east);
		\draw [arrow] ([yshift=-0.25cm]b7.west) -- ([yshift=-0.25cm]b6.east);

		
		%text at the top
		\node (nt1) at ($(b4.west)!0.5!(b7.east)$) {};

\draw [decorate,decoration={brace,amplitude=10pt,raise=25pt},xshift=0pt,yshift= 4cm]
(b4.west) -- (b7.east) node [black,midway,yshift=2cm] 
{\huge $\policy(\chain, B^\star_j) = \accept$};

\node [cloud, above of =b2, yshift = 4cm,draw,cloud puffs=10,cloud puff arc=120, aspect=2, inner ysep=3.6em](cl) { };
\node (cl1) [block, above of =cl, yshift =0.3cm]{\huge $B^\star_x$};
\node (cl2) [block, right of =cl1,xshift = 1cm,yshift =-0.8cm]{\huge $B^\star_y$};
\node (cl3) [left of =cl1,xshift = -1cm,yshift =-0.5cm]{\huge $\rcbpool$};
\node (cl4) [block, left of =cl,xshift = -0.3cm,yshift =-0.4cm]{\huge $B^\star_z$};

	\end{tikzpicture}
	}
\subcaption{After a successful voting phase, $B^\star_j$ replaces $B_j$ in the chain}
\label{fig:abstract_after_redaction}
\end{minipage}

\caption{The candidate block pool $\rcbpool$ stores the candidate blocks that are proposed and that can be endorsed in the voting phase. A block is linked to its predecessor by two links, the old link (solid arrow) and the new link (dashed arrow). In (a), a redact request $B^\star_j$ is proposed as a redaction for $B_j$ and added to $\rcbpool$, then the hash of $B^\star_j$ is included in the chain to denote a new candidate redaction; its voting phase starts just after its proposal. In (b), the candidate block $B^\star_j$ has gathered enough votes and was approved by the redaction policy $\policy$ of the chain; $B^\star_j$ replaces $B_j$ and the redacted chain is propagated. Note that new link from the block to the right of $B^\star_j$ is broken (marked by a cross), however the old link to $B^\star_j$ still holds. For simplicity, we consider the parameters $k=0$ (persistence), $\ell=4$ (voting period) and $\rho\ge 3/4$ (threshold for policy approval).}
\label{fig:abstract_protocol}
\end{figure*}

==> protocol.tex <==
\section{Editing the Blockchain}\label{sec:editing}
In this section we introduce an abstraction $\Blk$ of a blockchain protocol, and
we describe how to extend $\Blk$ into an \emph{editable} blockchain protocol
$\Blk'$.

%\TODOA{Need to say somewhere that we do one edit per block and it is easy to extend to more }
\subsection{Blockchain Protocol}\label{sec:abstract-new}


We consider an immutable blockchain protocol (for
instance~\cite{EC:GarKiaLeo15}), denoted by $\Blk$, where nodes receive inputs
from the environment $\env$, and interact among each other to agree on an
ordered ledger that achieves persistence and liveness. The blockchain protocol
$\Blk$ is characterised by a set of global parameters and by a public set of
rules for validation. 
The protocol $\Blk$ provides the nodes with the following set of interfaces
which are assumed to have complete access to the network and its users.

\begin{itemize}
\item $\{\chain',\bot\} \gets \Blk.\getChain$: returns a longer and \emph{valid}
    chain $\chain$ in the network (if it exists), otherwise returns $\bot$.

\item $\{0,1\} \gets \Blk.\chainValid(\chain)$: The chain validity check takes as input a chain $\chain$ and returns $1$ iff the chain is valid according to a public set of rules.

\item $\{0,1\} \gets \Blk.\blockValid(B)$: The block validity check takes as input a block $B$ and returns $1$ iff the block is valid according to a public set of rules. 

%\item $\Blk.\mkTx(\txType,\data)$: takes as input the transaction type information and the transaction data. It then constructs a transaction of type $\txType$ with data $\data$, validate the transaction and include it in the next block.

%%\item $\bit \gets \Blk.\isStbl(\chain, \data)$: takes as input a chain $\chain$ and some transaction data $\data$ and checks if the transaction containing $\data$ is \emph{stabilised} (w.r.t. the persistence property) in $\chain$. If yes, then it returns $1$, otherwise it returns $0$.

\item $\Blk.\broadcast(\data)$: takes as input some data $\data$ and broadcasts it to all the nodes of the system.
	
\end{itemize}

\noindent The nodes in the $\Blk$ protocol have their own local chain $\chain$
which is initialised with a common genesis block. The consensus in $\Blk$
guarantees the properties of persistence and liveness discussed
in~\cref{sec:blockchain_properties}.



%\subsection{Editable Blockchain}
%
%We build our editable blockchain protocol $\Blk'$ by modifying and extending the
%aforementioned protocol $\Blk$. The protocol $\Blk'$ has copies of all the basic
%blockchain functionalities exposed by $\Blk$ through the interfaces described
%above, and modifies the $\chainValid$ and $\blockValid$ algorithms in order to
%accommodate for edits in $\chain$. In addition, the protocol $\Blk'$ provides
%the following interfaces:
% \begin{itemize}
%	\item $\candidateblk_j \leftarrow \Blk'.\redactreq(\chain,j,\data^\star)$: takes as input the chain $\chain$, an index $j$ of a block to edit and some data $\data^\star$. It then returns a candidate block for $B_j$.
%
%	\item $\bit \leftarrow \Blk'.\decide(\candidateblk_j, \chain)$: takes as input a candidate block $\candidateblk_j$ and the chain $\chain$ and returns $1$ iff the candidate block $\candidateblk_j$ is valid.
% \end{itemize}
%
%The modified chain validation and block validation algorithms are presented
%in~\cref{alg:validate} and~\cref{alg:validateblk}, respectively, while the new
%algorithms to propose an edit to a  block and to validate candidate blocks are
%presented in~\cref{alg:request} and~\cref{alg:candidate}, respectively. In
%\cref{fig:protocol} we formally describe the protocol $\Blk'$.
%
%Intuitively, we need modifications for chain validation and block validation
%algorithms to account for an edited block in the chain. A block that has been
%edited possesses a different state, that does not immediately correlate with its
%neighbouring blocks. Therefore, for such an edited block we need to ensure that
%the old state of the block (the state before the edit) is still accessible for
%verification.\footnote{Note that the protocol does \emph{not} need to maintain
%the redacted data for verification, and therefore all redacted data is
%completely removed from the chain.} We do this by storing the old state
%information in the block itself. This therefore requires a modified block
%validation algorithm and a modified chain validation algorithm overall.
%
%
%
%We note that for simplicity our protocol is restricted to perform a single edit
%operation per block throughout the run of the protocol. In~\cref{apx:extension}
%we describe an extension of the protocol to accommodate for an arbitrary number
%of redactions per block.
%%The protocol is, however easily extendable to many edits per block if the block instead records all the state changes that ever occurred within that block's lifetime.
%
%
%\paragraph{Blockchain Policy}
%We introduce the notion of a blockchain policy $\policy$, that determines if an edit to the chain $\chain$ should be approved or not. The protocol $\Blk'$ is parameterised by a policy $\policy$ that is a function that takes as input a chain $\chain$ and a candidate block $\candidateblk$ (that proposes a modification to the chain $\chain$) and it returns $\accept$ if the candidate block $\candidateblk$ complies with the policy $\policy$, otherwise it outputs $\reject$; in case the modification proposed by $\candidateblk$ is still being deliberated in the chain $\chain$, then $\policy$ returns $\voting$. 
%
%In its most basic form, a policy $\policy$ requires that a candidate block $\candidateblk$ should only be accepted if $\candidateblk$ was voted by the majority of the network within some predefined interval of blocks (or \emph{voting period} $\ell$). A formal definition follows.
%
%%
%\begin{definition}[Policy]\label{def:policy}
%A candidate block $\editreq$ generated in round $r$ is said to satisfy the policy $\policy$ of chain $\chain := (B_1,\ldots,B_n)$, i.e., $\policy(\chain, \editreq) = \accept$, if it holds that $B_{r+\ell} \in \prune{\chain}{k}$ and the ratio of blocks between $B_r$ and $B_{r+\ell}$ containing $H(\editreq)$ (a vote for $\editreq$) is at least $\rho$, for $k,\ell \in \NN$, and $0 < \rho \le 1$, where $k$ is the persistence parameter, $\ell$ is the voting period, and $\rho$ is the ratio of votes necessary within the voting period $\ell$.
%\end{definition}
%
%
\restylefloat{figure}
\floatstyle{boxed}


\begin{figure*}
	The protocol $\layer$ has access to a blockchain protocol $\Blk$. The communication with $\Blk$ happens through the interfaces described in Section~\ref{sec:abstract-new}. The goal of $\layer$ is to extend $\Blk$ by acting as a layer that handles all the redact/edit operations. The protocol $\layer$ consists of a set of parties that can be categorised as \emph{miners, deciders} or \emph{users}. Note that the categories are \emph{not} mutually exclusive, e.g., an user can also be a decider and/or a miner. The protocol is parametrised by a policy $\policy$ that specifies the duration (in slot numbers) of the deliberation period. We formally describe the $\layer$ protocol below.
	
	\begin{flushleft}
		\textbf{Initialisation (miner).} Initialise the candidate blocks pool to be empty by setting $\rcbpool \gets \emptyset$.
	\end{flushleft}

	\begin{flushleft}
		\textbf{Proposal (user).} To propose an edit/redact request for the block $B_j:= \langle \header_j, x_j \rangle$, for $j \in [n]$, where $\header_j := \headerdesc{j}$, the user creates the candidate block $\candidateblk_j := \langle \header_j, x_j^\star \rangle$ with the new proposed data $x_j^\star$, and broadcasts it to the network by calling $\Blk.\broadcast(\candidateblk_j)$. Upon approval, the data contained in $x_j^\star$ will replace the data $x_j$ in the blockchain; if the proposal is to redact (i.e. to purge) the contents of $x_j$ then $x_j^\star = \emptyset$. 
	\end{flushleft}

	\begin{flushleft}
		\textbf{Update pool (miner).} The blockchain miners periodically collect all candidate blocks $\candidateblk_j$ from the network and add $\candidateblk_j$ to the pool of candidate blocks
		$\rcbpool$ iff the candidate block $\candidateblk_j$ is valid in respect to the current chain $\chain \gets \Blk.\getChain$; otherwise discard $\candidateblk_j$.
	\end{flushleft}

	\begin{flushleft}		
		\textbf{Deliberation (decider).} For all candidate blocks $\candidateblk_j \in \rcbpool$, the deciders can deliberate and scrutinize $\candidateblk_j$ to decide whether they support the proposal or not; they can cast their vote $\vote$ (either accept or reject) by invoking $\Blk'.\deliberate(\candidateblk_j, \vote)$. \emph{After} the deliberation period specified by the policy $\policy$ has elapsed, the protocol $\layer$ outputs a final decision $\decision_j:= (j, b, G(s_j,x_j), x^\star_j)$, where $b=1$ if the decision is to approve the modification and $0$ otherwise, and stores $\decision_j$ in the blockchain $\Blk$. Note that the final decision $d_j$ can be an arbitrary function of the votes of the deciders, e.g., $d_j$ represents the majority of the votes casted for $\candidateblk_j$. The final decision $d_j$ for each $\candidateblk_j$ that was in $ \rcbpool$ can be retrieved by invoking $d_j \gets \Blk'.\getDecision(\chain, \candidateblk_j)$; if $d_j=\emptyset$ then the decision $d_j$ does not yet exist.
	\end{flushleft}

	\begin{flushleft}		
		\textbf{Editing the chain (miner).} Before extending the chain and creating the next block $B_{i}$, for all candidate blocks $\candidateblk_j \in \rcbpool$, where $j<i$, check if there is a final decision for the request $\candidateblk_j$ by invoking $\decision_j \gets \Blk'.\getDecision(\chain, \candidateblk_j)$; if $d_j \ne \emptyset$ then remove $\candidateblk_j$ from $\rcbpool$, and if the decision $\decision_j$ is to accept the request, then proceed as follows.
			\begin{itemize}
				\item \emph{Redaction (stateless update)}: In this case, the miners replace $B_j$ with $\candidateblk_j$ in the chain and extend the chain with the new block $B_i$ as usual. No further change is needed as none of the other blocks are affected.
				\item \emph{Stateful update}: In case of stateful updates, the miners use the $\layer$ state transition function $\hat{x}_{i}:=\transition^\star(\chain,d_j,x_{i})$, where $x_{i}$ is the incoming data for the current round $i$, to create the data $\hat{x}_{i}$ that updates the state according to the decision $d_j$. Then, create the new block $B_{i} := \langle \header_{i}, \hat{x}_{i}||x_i \rangle$, where $\header_{i}:=(s_{i},G(s_{i},\hat{x}_{i}||x_i), \pi_{i})$ and append it to the chain $\chain$. 
			\end{itemize}
		 
	\end{flushleft}
	
		\begin{flushleft}
		\textbf{Validating chain edits (miner).} 
%		A candidate block $\candidateblk_j$ can be proposing one of two different types of modifications, namely \emph{redaction}, where data is removed from the chain but no future transactions (and state) are affected, or \emph{state update} where the data does not get removed but the state of the chain gets updated to reflect the proposed modification. 
The chain validation is performed as in $\Blk$ by validating blocks starting from the genesis, and only if there is an accepting decision $d$ in the chain that the $\layer$ protocol intervenes. We detail this intervention next: 
For each accepting decision $d_j \in \chain$ included in block $B_i$, miners retrieve the candidate block $\candidateblk_j$ that was approved by $d_j$ by invoking $\candidateblk_j \gets \Blk'.\getCandidate(\chain,d_j)$. Then, according to $\candidateblk_j$ one of the following validation procedures happen. 
		\begin{itemize}
			\item \emph{Redaction (stateless update)}:  In the case of a redaction, the data $x_j$ that was part of $B_j$ was removed. Therefore, to successfully validate such a redacted block, miners will have to verify that the decision $d_j$ contains the correct value $G(s_j,x_j)$, that is included in the header of the block $\candidateblk_j$ in the chain. One also checks if the hash links hold between the headers of $B_j$ and $B_{j+1}$ with $G(s_j,x_j)$. In that case, the redaction was approved and the redacted block should be considered valid.
			 
			\item \emph{Stateful update}: In case of a stateful update, %
			%we have that $\transition(\pruneclose{\chain}{i-1},x_i)\ne \transition(\pruneclose{\chain_1}{i-1},x_i)$ where $\chain_1 = \pruneclose{\chain}{j-1}||\candidateblk_j||\pruneback{\chain}{j}$, i.e., it is the chain where the candidate block replaces the original block. 
miners check if $\hat{x}_{i+1} = \transition^\star(d_j,\pruneclose{\chain}{i},x_{i+1})$ where $x_i$ was the incoming data for the $i$-th block that can be retrieved from $B_i$ and $\transition^\star$ is the state function of the $\layer$ that performs state updates after an edit operation. In the affirmative case accept the block as valid.
		\end{itemize}
	\end{flushleft}

%	\begin{flushleft}
%		\textbf{Validating the chain (miner).} If validating the chain according to $\Blk.\chainValid(\chain)$ fails by outputting $0$ due to an error at block $B_i = \generalheaderi{i}||\left\langle \parsex{i}{}\right\rangle$, $\miner$ does the following:
%		\begin{enumerate}
%			\item In case some purge happened at this block, check if $\getDecision(\chain,x_i)$ is an accept. In this case the decision process would have happened after block $B_i$ was mined.
%			\item In case state transition does not hold from block $i-1$ to $i$, that is $\transition(\chain,\pruneclose{\edit}{i},x_i)\ne y_i$, check the approved list $\edit_i$ and retrieve $x_j^\star$ that was approved at this point. Check if $\getDecision(\chain, x_j^\star)$ is an accept. Now verify if the state transition from $i-1$ to $i$ after the approved edit operation, by checking if $\transition^\star(\chain,\pruneclose{\edit}{i}, x_j^\star, x_i) = y_i$.
%			\item If any of the above checks or retrievals output $0$ or $\emptyset$ respectively, discard the chain as invalid and output $0$.
%		\end{enumerate}
%	\end{flushleft}
	
%		\MESSAGEB{This is a first shot at abstracting the generic protocol. Still to be done: \begin{itemize}
%			\item Parametrize with the Policy
%			\item Rewrite the $\editchain$ algorithm
%			\item Match the underlying blockchain interface to this
%			\item Match the instantiations to this protocol (most of the consensus-specific complexity will go to the instantiations)
%	\end{itemize}}
	\caption{Accountable permissionless editable blockchain protocol $\Blk'_\policy$}
	\label{fig:protocol}
\end{figure*}

\subsection{Protocol Description}\label{sec:protocol}
We denote a block to be of the form $B:= \langle \header, x \rangle$, with $\header:=\headerdesc{}$ where $s \in \bit^\spar$ is the hash of the previous block, $s:=H(\poc,G(s,x))$, $x \in \bit^*$ is the block content, and $\poc \in \{ 0,1\}^\spar$ is the proof of consensus. Here $x$ denoting the data included into the block coming from the network and the state information of the system until that point. 

The block validation procedure $\Blk.\blockValid(B)$ checks if the hash links $s$ in its header is the hash of the previous header, if the information $G(s,x)$ corresponds to the data stored in the block and finally if the consensus proof $\poc$ is correct according to $\chain$ and its rules. The chain validation procedure $\Blk.\chainValid(\chain)$ checks if every block in $\chain$ is valid based on the above mentioned checks. 

Our protocol for performing edit operations acts as a layer on top of the existing blockchain protocol $\Blk$. Our $\layer$ takes care of the necessary operations and validation procedures that concern with edit operations while letting the procedures in $\Blk$ carry on without any other interferences. 

\paragraph{Intuition} On a high level the $\layer$ classifies the users of system as \emph{miners, deciders} and \emph{users}. Any \emph{user} is allowed to make an edit request that can either purge some data from a block or perform an edit operation that changes the state of the system from thereon. A \emph{miner} collects all such requests from the network and validates them before adding them to the candidate pool of candidate blocks. If a request is approved, the \emph{miner} performs the edit operation, be it purging of data or a stateful edit operation. In case of stateful edits, the \emph{miner} also needs to update the state of the system starting from the position the edit was performed until the point the request has been approved. To do this, we introduce the $\layer$ state transition function $\transition^\star: \bit^* \times \bit^* \times \bit^* \rightarrow \bit^*$ that takes as inputs the latest approved request, the chain and the new inputs from the network and returns the updated state of the system until that point in time. $\transition^\star$ takes into account the all the previous state updates that are reflected onto the chain already. \emph{Decider} deliberate on a proposed request and vote for the request to be approved or not. If the votes satisfy the edit policy $\policy$ of the system, then the request is considered to be approved and a decision $d$ is posted on the blockchain that helps \emph{miners} perform the edit operation and also future users in validation of chain edits.





During the setup of the system, the chain $\chain$ is initialised as $\chain:=\genesis$, and all the users in the system maintain a local copy of the chain $\chain$ and a pool $\rcbpool$ consisting candidate blocks for edits, that is initially empty. The protocol runs in a sequence of rounds $\round$ (starting with $\round := 1$). 


%\floatstyle{plain}
%\restylefloat{figure}
%\begin{figure}
%\centering
%\begin{tabular}{p{.40\columnwidth} p{.46\columnwidth}}
%\textbf{Value} & \textbf{Description} \\ \thickhline
%$\mathtt{state\_link}\ (s)$ & link to the previous block\\ \hline
%$\mathtt{data}\ (x)$ & data items stored in the block\\ \hline
%$\mathtt{counter}\ (\ctr)$ & proof of mining the block correctly\\ \thickhline
%%$\mathtt{timestamp}$ & the timestamp of the block \\ \hline
%%%$\mathtt{nonce}$ & nonce used in proof-of-work \\ \thickhline
%\rowcolor{Gainsboro!30}$\mathtt{old\_state}\ (y)$ & original state of the block when created $(=G(s,x))$\\ \thickhline
%
%\end{tabular}%}
%\caption{Structure of the block $B$. The last highlighted field ($\mathtt{old\_state}$) is only included in the block of the extended (editable) protocol. A candidate block $B^\star$ for $B$ is of the form $(s,x^\star,\ctr,y)$ where only the data stored has been edited.}
%\label{fig:modifyblockabstract}
%\end{figure}


%In the beginning of each round $\round$, the users try to extend their local chain using the interface $\Blk'.\getChain$, that tries to retrieve new valid blocks from the network and append them to the local chain. Next, the users collect all the candidate blocks $\candidateblk_j$ from the network and validate them by using $\Blk'.\decide$ (\cref{alg:candidate}); then, the users add all the valid candidate blocks to the pool $\rcbpool$. 
%For each candidate block $\candidateblk_j$ in $\rcbpool$, the users compute $\policy(\chain,\candidateblk_j)$ to verify if the candidate block $\candidateblk_j$ should be adopted by the chain or not; if the output is $\accept$ they replace the original block $B_j$ in the chain by the candidate block $\candidateblk_j$ and remove $\candidateblk_j$ from $\rcbpool$. If the output is $\reject$, the users remove the candidate block $\candidateblk_j$ from $\rcbpool$, otherwise if the output is $\voting$ they do nothing. 
%To create a new block $B$ the users collect transactions from the network and store them in $x$; if a user wishes to endorse the edit proposed by a candidate block $\candidateblk_j \in \rcbpool$ that is still in $\voting$ stage, the user can vote for the candidate block $\candidateblk_j$ by simply adding $H(\candidateblk_j)$ to the data $x$. After the block is created and the new extended chain $\chain':= \chain||B$ is built, the users broadcast the new chain $\chain'$ iff $\Blk'.\chainValid(\chain') = 1$ (\cref{alg:validate}). 
%Finally, if a user wishes to propose an edit to block $B_j$ in the chain $\chain$, she first creates the new data $x^\star_j$, that represents the modifications that she proposes to make to the data $x_j$, and calls $\redactreq$ (\cref{alg:request}) using the interface $\Blk'.\redactreq$ with the chain $\chain$, index $j$ of the block in $\chain$ and the new data $x^\star_j$. The algorithm returns a candidate block $\candidateblk_j$ that is broadcasted to the network.


%%%%%%%%%% Validate chain
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Chain Validation} 
%
%\begin{algorithm}
%\SetAlgoVlined
%\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\Input{Chain $\chain = (B_1,\cdots,B_n)$ of length $n$, and their tails $\Tail = (\Tail_{B_1},\cdots,\Tail_{B_n})$.}
%\Output{$\bit$}
%
%\BlankLine
%Initialise set $\editset = \emptyset$\;
%$j=2$\;
%\While{$j \le n$}{
%Parse $B_j := \generalblocki{j}$\;
%Parse $\Tail_{B_j}:= \Taili{j}$\;
%\lIf{$\Blk'.\blockValid(\prune{\chain}{n-(j-1)},\prune{\Tail}{n-(j-1)},B_j,\Tail_{B_j})=0$}{\Return $0$}
%\lIf{$G_1(s_j,x_j) \ne G_1(s_{\old,j},x_{\old,j})$}{\newline
%Set $\editset = \editset \cup \{ h(j,B_j) \}$}
%j=j+1\;
%}
%Set $\approvedset = \{ h(i,B_i) |\ \policy(\chain,h(i,B_i))=\accept,h(i,B_i)\in \chain \}$\;
%\lIf{$\editset \ne \approvedset$}{\Return $0$}
%\lElse{\Return $1$}
%\caption{$\chainValid$ \footnotesize{(implements $\Blk'.\chainValid$)}}	
%\label{alg:validate}
%\end{algorithm}
%
%
%%%%%%%%%% Validate block
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Block Validation}    
%
%\begin{algorithm}
%\SetAlgoVlined
%\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\Input{Chain $\chain = (B_1,\cdots,B_n)$, tails $\Tail = (\Tail_{B_1},\cdots,\Tail_{B_n})$, block $B$ and its tail $\Tail_B$.}
%\Output{$\bit$}
%
%\BlankLine
%Parse $B := \generalblock$, where $x:=(X,Y)$\;
%Parse $\Tail_B := (\poc_{\old},s_{\old},G(s_\old,x_\old))$\;
%Parse $B_n := \generalblocki{n}$\;
%Parse $\Tail_{B_n} := \Taili{n}$\;
%Validate data $X$, if \emph{invalid} \Return $0$\;
%\lIf{$Y \ne \transition(x_n,X)$}{\Return $0$}
%\uIf{$s=H(\poc_n,G(s_n,x_n))$}{ 
%\lIf{$ \checkconsensus(\chain,(\poc,G(s,x))) \lor \checkconsensus(\chain, (\poc_\old,G(s_\old,x_\old))) $}{\Return $1$}}\label{line:pow}
%\uElseIf{$s=H(\poc_{\old,n},G(s_{\old,n},x_{\old,n})) \land \checkconsensus(\chain, (\poc_\old,G(s_\old,x_\old)))$}{\Return $1$}
%\lElse{\Return $0$}\label{line:ret}
%\caption{$\blockValid$ \footnotesize{(implements $\Blk'.\blockValid$)}}	
%\label{alg:validateblk}
%\end{algorithm} 
%
%%%%%%%% Requesting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Proposing an Edit} 
%
%\begin{algorithm}
%  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%   \Input{Chain $\chain = (B_1,\cdots,B_n)$ of length $n$, an index $j \in [n]$, and the new data $\newdata_j^\star$.}
%  \Output{A candidate block $\candidateblk_j$.}
%  \BlankLine 
%    Parse $B_j:= \generalblocki{j}$\;
%    Parse $B_{j-1} := \generalblocki{j-1}$\;
%    Build the candidate block $\candidateblk_j := \langle s_j,(\newdata_j^\star,\transition(x_{j-1},\newdata_j^\star)),\poc_j\rangle$\;
%    \Return $\candidateblk_j$\;
% \caption{$\redactreq$ \footnotesize{(implements $\Blk'.\redactreq$)}}
% \label{alg:request}
%\end{algorithm}
%
%%%%%%%%%% Candidate block validating
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Validating Candidate Blocks} 
%
%\begin{algorithm}
%	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\Input{Chain $\chain = (B_1,\cdots,B_n)$ of length $n$, and a candidate block $\candidateblk_j$ for an edit.}
%\Output{$\bit$}
%\BlankLine
%Parse $\candidateblk_j := \langle s^\star,x^\star,\poc^\star\rangle$, where $x^\star := (X^\star,Y^\star)$\;
%Parse $B_{j}:= \generalblocki{j}$\;
%Parse $B_{j-1}:= \generalblocki{j-1}$\;
%Validate data $X^\star$, if \emph{invalid} \Return $0$\;
%\lIf{$s^\star = s_j \land Y^\star = \transition(x_{j-1},X^\star) \land \poc^\star = \poc_j$}{\Return $1$}
%\Return $0$\;
%
%\caption{$\decide$ \footnotesize{(implements $\Blk'.\decide$)}}
%\label{alg:candidate}
%\end{algorithm}
%
%%%%%%%%%% Editing the chain
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Editing the chain}
%
%\begin{algorithm}
%	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\Input{Chain $\chain = (B_1,\cdots,B_n)$ of length $n$, tails $\Tail = (\Tail_{B_1},\cdots,\Tail_{B_n})$, and a candidate block $\candidateblk_j$ for an edit.}
%\Output{chain $\chain'$}
%\BlankLine
%Initialize $i = j+1,\chain^\star = \emptyset$\;
%Set $B_j = B_j^\star$\; 
%\While{$i \le n$}{
%Parse $\Tail_{B_i}:=\Taili{i}$\;
%Parse $B_i := \generalblocki{i}$ and $B_{i-1} := \generalblocki{i-1}$, where $x_i := (X_i,Y_i)$\;
%Set $B_i \gets \langle s_{\old,i},(X_i,\transition(x_{i-1},X_i)),\poc_{\old,i}\rangle$\;
%Set $\chain^\star \gets \chain^\star \vert\vert B_i$\;
%}
%Set the updated chain $\chain' \gets \prune{\chain}{n-(j-1)}\vert\vert \candidateblk_j \vert\vert\chain^\star$\;
%\Return $\chain'$\;
%\caption{$\editchain$ \footnotesize{(implements $\Blk'.\editchain$)}}
%\label{alg:editchain}
%\end{algorithm}




